Evaluating Distributed Representations for Multi-Level Lexical Semantics: A Research Proposal

Modern neural networks (NNs), trained on extensive raw sentence data, construct distributed representations by compressing individual words into dense, continuous, high-dimensional vectors. These representations are expected to capture multi-level lexical meaning. In this thesis, our objective is to examine the efficacy of distributed representations from NNs in encoding lexical meaning. Initially, we identify and formalize three levels of lexical semantics: \textit{local}, \textit{global}, and \textit{mixed} levels. Then, for each level, we evaluate language models by collecting or constructing multilingual datasets, leveraging various language models, and employing linguistic analysis theories. This thesis builds a bridge between computational models and lexical semantics, aiming to complement each other.

==> main/2_Related_work.tex <==
\section{Related Work}
\label{related work}

\subsection{Interpretability of language models}
% Researchers aim to understand the inner workings of language models and their learning process, which is often seen as a black-box due to the end-to-end pipeline in deep learning. 
Interpretability of LLMs can be categorized into mechanistic (bottom-up) and representational (top-down) analysis~\cite{zou2023representation}. Mechanistic interpretability focuses on translating model components into understandable algorithms for humans, typically by representing models as computational graphs and identifying circuits with specific functions~\cite{mecha_olsson2022context,graph_geiger2021causal,function_wang2022interpretability}. On the other hand, representational analysis abstracts away lower-level mechanisms and explores the structure and characteristics of representations. Probing, an effective approach in top-down interpretability, can be classifier-based or geometric-based. Classifier-based probing trains additional classifiers for specific proxy tasks, including syntactic analysis~\cite{hewitt2019syntax}, semantic roles~\cite{semantic_roles_ettinger2020bert}, named entity recognition~\cite{ner2023gpt}, and world knowledge~\cite{world_petroni2019language}. These linguistic features have demonstrated a rich hierarchy, spanning from lower layers to higher layers~\cite{jawahar-etal-2019-bert-hierachy}.
% but suffers from additional parameters and task designations. 
Geometric probing without additional classifiers, examines the properties of the representational space itself. For example, difference vectors, obtained by subtracting base vectors, can detect linguistic features such as scalar adjective intensity~\cite{gari-soler-apidianaki-2021-scalar} and stylistic features~\cite{stylistic_lyu-etal-2023-representation}. 
% Moreover, transformations in the vector space, like principal component analysis (PCA) and independent component analysis (ICA), reveal semantic information~\cite{ica_yamagiwa-etal-2023-discovering}. These probing experiments often come with layer-wise performance. 
Furthermore, methods from the view of information flow indicate that models with autoregressive objectives~\cite{voita-etal-2019-bottom} and specifically LLMs~\cite{wang-etal-2023-label} gather information in shallow layers while making predictions in deep layers.

\subsection{Representations of Lexical Semantics}
Lexical semantics, the study of word meanings, is a prominent field in both linguistics and computational research. Linguistics offers rich descriptive entries, known for their high dimensionality, contextual modulation, and discreteness~\cite{break-petersen-potts-2023-lexical}. Early rule-based models, including the Generative Lexicon~\cite{pustejovsky1998generative} approach, used discrete feature representations. In contrast, neural models represent words as compact continuous vectors to avoid arbitrary feature selection. Static vector models, such as word2vec~\cite{word2vec}, Glove~\cite{pennington-etal-2014-glove}, and fastText~\cite{fasttext}, provide unified representations for all word occurrences. To distinguish word meanings in various contexts, especially for polysemous words, researchers have developed context-sensitive representations. Notable models include Elmo~\cite{elmo-peters-etal-2018-deep}, BERT~\cite{kenton2019bert}, and the GPT family~\cite{gpt2,gpt3}. While LSTM-based Elmo and transformer-based models offer bidirectional context around the target word, the GPT family focuses solely on context preceding the query word as a generative model. Large language models (LLMs)~\cite{touvron2023llama, gpt3} follow training mechanisms similar to GPT and have shown competitive performance via prompting engineering~\cite{white2023prompt} compared to BERT-like models, e.g., in lexical tasks like word sense disambiguation~\cite{wsd-kocon2023chatgpt} and named entity recognition~\cite{ner2023gpt}. Our research emphasizes evaluating the quality of representations in LLMs to enhance interpretability, rather than focusing on prompting strategies.


==> main/5_Results.tex <==
\section{Results and Analysis}
\label{sec: results}
% \subsection{Overall Comparison}
\begin{table}[t]
    \centering
    \small
    % \setlength{\tabcolsep}{0.6 mm}{
    \begin{tabular}{cccc}
    \toprule
        Method & All & Noun & Verb\\
        \midrule
        Human & 80.0 & - & - \\
        Random & 50.0 & - & - \\
        \midrule
        WSD & 67.7 & - & - \\
        BERT\_large\dag (23) & 67.8 & 69.1 & 67.6 \\
        BERT\_large (22) & \textbf{71.0} & \textbf{70.7} & \textbf{71.5} \\
        Context2vec & 59.3 & - & - \\
        Elmo & 57.7 & - & - \\
        \midrule

        Llama2\_base\dag (6) & 60.9 & 62.6 & 62.1 \\
        Llama2\_base (12) & 62.9 & 63.9 & 62.5 \\
        Llama2\_repeat\dag (8) & 64.6 & 66.5 & 63.6 \\
        Llama2\_repeat (7) & 68.4 & \underline{70.3} & 65.5 \\
        Llama2\_prompt\dag (23) & 68.9 & 68.9 & \underline{69.5} \\
        Llama2\_prompt (20) & \underline{69.2} & 69.2 & \underline{69.5} \\

        \bottomrule
    \end{tabular}
    % }
    \caption{Overall accuracy (\%) on the WiC test set. \dag indicates methods without anisotropy removal. The numbers in brackets after the model name indicate the number of layers for achieving the best performance.}
    \label{tab:overall}
\end{table}
Table~\ref{tab:overall} presents the overall performance. Llama2, as a generative model, achieves comparable results to bidirectional and non-regressive BERT models, outperforming non-transformer models like Elmo. This suggests that LLMs have the potential for word-level understanding, even though it is not explicitly trained for this capability. As expected, the prompting strategy achieves the highest accuracy among all the Llama2 variants. This approach incorporates downstream tasks into the generative process during LLM training and has proven to be popular and effective in addressing both intermediate and high-level tasks in the LLM era~\cite{zhao2023survey}. However, prompting relies on the choice of prompts and may not directly reveal the model's internal understanding. On the other hand, our repeat strategy demonstrates comparable performance to prompting and significantly outperforms the base version (with a 5.5 advantage gap). This simple yet effective transformation strikes a balance between information accessibility and prompting robustness.

In terms of parts-of-speech, nouns generally exhibit higher accuracy than verbs, as evidenced by a 4.8 advantage gap in Llama2\_repeat. This observation aligns with previous studies that have concluded that verbs are more challenging to disambiguate \cite{verb-barba-etal-2021-consec}.

% \subsection{\textcolor{blue}{Ablation Study}}
\paragraph{Effectiveness of Anisotropy Removal.} In Table~\ref{tab:overall}, we compare methods with and without anisotropy removal (marked by \dag). The results consistently demonstrate the advantage of methods with anisotropy removal, suggesting that the representation space may collapse into a smaller cone space, as indicated by previous work \cite{ethayarajh2019contextual}. This also offers a simple and practical approach for calculating similarity in the embedding space.

\begin{figure}[h]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/v2_layer_wise.pdf}
    \caption{Layer-wise accuracy for different settings and models. Star shows the best value.}
    \label{fig:layer_wise}
\end{figure}


\paragraph{Trends Across Layers.} Figure~\ref{fig:layer_wise} illustrates the layer-wise dynamics in two settings for Llama2 and also BERT\_large. We observe non-monotonic trends for Llama2 across layers: both the base and repeat initially increase in lower layers before decreasing in higher layers. Consequently, optimal performance is achieved at lower layers when utilizing the hidden states of the target word as the default choice. This suggests that lower layers in LLMs encode lexical semantics, offering both a practical insight and a pathway for interpreting LLMs. Moreover, the trend contrasts with bidirectional BERT\_large model, which obtains the best performance in higher layers. This highlights a difference between these two architectures: BERT concentrates on its current word across the layers while Llama2 aims for next token prediction. 
% These results have important implications for the design and interpretation of LLMs, and contribute to a deeper understanding of their underlying mechanisms.


% This observation may stem from LLMs being trained with an objective of next token prediction, wherein higher layers closer to the classification head tend to capture semantic features of the subsequent predicted tokens rather than the current tokens. This phenomenon is supported by the prompting strategy, where the punctuation itself does not carry the meaning of the target word; instead, the next token is prompted to represent the word's meaning. As a result, higher layers yield optimal results in this scenario.

\begin{figure}[h]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/v2_prediction.pdf}
    \caption{Layer-wise accuracy of Llama2 representations (repeat and prompt setting), as well as the previous token in the repeat setting (repeat\_prev). The increasing trends observed in repeat\_prev and prompt accuracies, as well as the non-monotonic trend observed in repeat accuracy, suggest that while the understanding ability may be weakening, the predictive ability is improving.}
    \label{fig:ntp_comp}
\end{figure}

\paragraph{Balancing Understanding and Prediction.} 
To explore the balance between lexical understanding and predictive capability in Llama2, we computed the accuracy using representations of the previous token before the target (referred to as repeat\_prev) in the repeat setting. It is important to note that we opted for the repeat setting instead of the base setting, given that the base setting is constrained by incomplete information access. Furthermore, we conducted a comparison with the prompt setting, as depicted in Figure~\ref{fig:ntp_comp}. Despite the fact that the representations do not originate from the correct target word but are anticipated to represent the next word, both repeat\_prev and prompt exhibit a monotonic trend and comparable result across the layers. This observation suggests that while the understanding may diminish (as indicated by the inverted-U trend in the repeat setting) as layers go deeper, the predictive ability improves.

% In order to examine the trade-off between lexical understanding and predictive ability in Llama2's higher layers, we evaluate its predictive accuracy across layers in the repeat setting, as illustrated in Figure~\ref{fig:ntp_comp}. We achieve this by extracting the classifier parameter $W$ from the end of Llama2 and applying it to the hidden states of each layer. After normalization using softmax, we consider the probability of the next token as the predictive accuracy.

% As depicted by the red line and right axis in Figure~\ref{fig:ntp_comp}, Llama2 exhibits an increasing predictive capability alongside a decreasing understanding ability in higher layers. This is because Llama2 is predominantly optimized for the objective of next token prediction, with representations at the highest layer directly used for this purpose. In contrast, BERT-like architectures integrate both understanding and prediction since their objective involves restoring or predicting the current word. As a result, BERT-like models demonstrate a monotonically increasing accuracy in understanding the target word, as shown in Figure~\ref{fig:ntp_comp}.
